AppealMod: Inducing Friction to Reduce Moderator Workload of Handling User Appeals

As content moderation becomes a central aspect of all social media platforms and online communities, interest has grown in how to make moderation decisions contestable. On social media platforms where individual communities moderate their own activities, the responsibility to address user appeals falls on volunteers from within the community. While there is a growing body of work devoted to understanding and supporting the volunteer moderators' workload, little is known about their practice of handling user appeals. Through a collaborative and iterative design process with Reddit moderators, we found that moderators spend considerable effort in investigating user ban appeals and desired to directly engage with users and retain their agency over each decision. To fulfill their needs, we designed and built AppealMod, a system that induces friction in the appeals process by asking users to provide additional information before their appeals are reviewed by human moderators. In addition to giving moderators more information, we expected the friction in the appeal process would lead to a selection effect among users, with many insincere and toxic appeals being abandoned before getting any attention from human moderators. To evaluate our system, we conducted a randomized field experiment in a Reddit community of over 29 million users that lasted for four months. As a result of the selection effect, moderators viewed only 30% of initial appeals and less than 10% of the toxically worded appeals; yet they granted roughly the same number of appeals when compared with the control group. Overall, our system is effective at reducing moderator workload and minimizing their exposure to toxic content while honoring their preference for direct engagement and agency in appeals.

==> tables/descriptive-stats.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
                                                           & Control & Treatment & Total \\ \hline
Total appeals                                              & 438     & 442       & 880   \\ \hline
Appeals that completed screening process                   & —       & 131       & 131   \\ \hline
Appeals that moderators responded to                       & 263     & 105       & 368   \\ \hline
Follow up conversations between users and human moderators & 162     & 84        & 246   \\ \hline
Accepted appeals                                           & 48      & 42        & 90    \\ \hline
\end{tabular}

\caption{Summarizing the data collected during the experiment period}
\label{tab:descriptive-stats}
\end{table}

==> tables/historical-data.tex <==
\begin{table}[]
\begin{tabular}{|l|r|}
\hline
Banned Users                        & 16262 \\ \hline
Ban Appeals                         & 6543  \\ \hline
Appeals with follow-up conversation & 2859  \\ \hline
Appeals accepted                    & 846   \\ \hline
\end{tabular}
\vspace{8px}
\caption{Historical data for 2021 (collected before the experiment period) }
\label{tab:historical-data}
\end{table}
